War Elephants: Rethinking Combat AI and Human Oversight

This paper explores the changes that pervasive AI is having on the nature of combat. We look beyond the substitution of AI for experts to an approach where complementary human and machine abilities are blended. Using historical and modern examples, we show how autonomous weapons systems can be effectively managed by teams of human "AI Operators" combined with AI/ML "Proxy Operators." By basing our approach on the principles of complementation, we provide for a flexible and dynamic approach to managing lethal autonomous systems. We conclude by presenting a path to achieving an integrated vision of machine-speed combat where the battlefield AI is operated by AI Operators that watch for patterns of behavior within battlefield to assess the performance of lethal autonomous systems. This approach enables the development of combat systems that are likely to be more ethical, operate at machine speed, and are capable of responding to a broader range of dynamic battlefield conditions than any purely autonomous AI system could support.

==> text2/AI_problems.tex <==
\subsection{AI Limitations}
\label{sec:ai_problems}

AI is largely a way of transforming one set of patterns (e.g. words, such as \enquote{black and white animation cell showing steamboat willie sitting at a computer}) into another set of patterns, such as the image in Figure~\ref{fig:steamboat_willie}:

\begin{figure}[htbp]
    \centering
    \fbox{\includegraphics[width=0.5\linewidth]{figures/steamboat.png}}
    \caption{MidJourney Rendering}
    \label{fig:steamboat_willie}
\end{figure}

A less frivolous example would be to transform radar returns into actionable insights such as firing recommendations. It is up to the AI developer to define the parameters of the domain of that transformation. AI can sometimes provide insights to enable better decision making, but it cannot be trusted to provide solutions that make sense outside of its training.

AI systems are often excellent at working in constrained contexts, but they may not be able to handle more complex or dynamic situations. For example, a chess AI may be able to beat a human player in a game of chess, but it may not be able to handle a game with changing rules or a game of 3D chess when it has been trained on the traditional 8x8 board.

Human beings have a different set of capabilities and deficits. We can learn and adapt on the fly, but get bored and distracted. We can think outside of the box, but we are biased and make mistakes. We are capable of making rapid decisions in the face of uncertainty, but in situations that require deliberation, we can become overwhelmed or paralyzed.

Humans can provide the judgment and intuition to help guide AI-driven decisions, but they can also be manipulated or biased by the very systems they are working with. As AI becomes more commonplace, it is important to consider both the potential benefits and the potential risks. If an AI system makes a decision which fails to take into account all relevant factors such as human values, ethical principles and legal frameworks, then it may run the risk of making poor decisions with catastrophic consequences. Let's look in detail at the limitations of AI and Human capabilities and how they can be addressed. 

\subsubsection{Inherent limitations with Narrow AI}
\label{sec:narrow_ai}

% There is no doubt that the python code in Listing~\ref{eq:number_str} will \textit{always} create a character string \textit{only} containing a sequence of comma-separated numbers with a given starting point of any desired length. The drawback is that the deterministic system is limited to its designed task and is incapable of responding outside of that very narrow scope. 

% \begin{equation}
%     \texttt{s = ', '.join(map(str, range(start, start+length)))}
%     \label{eq:number_str}
% \end{equation}

% The power of deep learning is that the same system that can extend a sequence of numbers can also extend any other text. 

\begin{comment}
AI struggles with \textit{sequences} of patterns, or more simply, \textit{time}. For example, when given the prompt \enquote{a photograph of a ball falling at 1, 2, and 3 seconds,} a state-of-the-art image generation program such as DALL-E can create a set of beautifully rendered balls that are clearly \textit{not} falling, as shown in Figure~\ref{fig:falling_ball}. Specialized architectures such Recurrent Neural Networks (RNN) and Long-Short-Term-Models (LSTMs) exist so that neural networks can learn patterns over time, but they are not as efficient or scalable as other architectures such as Transformers. Even the groundbreaking Transformer architecture struggles with understanding sequential events. Indeed, the Transformer architecture has to include an additional \textit{positional encoding} component to provide sequential information.

\begin{figure}[!htbp]
	\centering
    \begin{subfigure}{.45\textwidth}
        \centering
    	\fbox{\includegraphics[height=15em]{figures/ball_falling_at_1_2_and_3_seconds}}
    	\caption{\label{fig:falling_ball} Best SD result after multiple attempts}
    \end{subfigure}
        \begin{subfigure}{.45\textwidth}
        \centering
    	\fbox{\includegraphics[height=15em]{figures/ball_falling}}
    	\caption{\label{fig:falling_ball_search} First Google Image Search result\footnotemark}
    \end{subfigure}
    \caption{Text-to-image vs. Search}
\end{figure}
\footnotetext{The reason that search is better in this instance is because most search engines use a process that changes a query to a position in high-dimensional space and then searches for the closest document of the desired type that is \enquote{closest} to the query in that space.}
\end{comment} 
Many of the applications where we interpret AI as \textit{thinking ahead}, are actually examples of seeing deep patterns \textit{in the moment}. Gary Kasparov described this process where chess computers \enquote{rate as many variations as possible in the given position and puts a value on each position it sees. The move that returns the highest value is put at the top of its move list as the move to make.} In opposition to this approach is the human approach, which views chess play as a kind of narrative where \enquote{players would fall into the trap of seeing each game of chess as a story, a coherent narrative with a beginning and a middle and a finish.}~\parencite{kasparov2017deep} 

Even Large Language Models (LLMs) such as the GPT-3, which are capable of writing compelling narratives are pattern matching in the moment. In this case, some number of preceding tokens is used to calculate the probability of the next token, be it word, space, or punctuation. That token is in turn added to the input and the process repeats. That the process so accurately reflects human writing says more about the latent pattern in our writing than it may about the ability for a machine to tell a compelling story~\parencite{brown2020language}.

\TODO{Introduce LLM hallucinations here} 

Good predictions involving time can be made where large amounts of consistent data are available, such as physics modeling using recurrent neural network (RNN) approaches. But these models are highly constrained to make quality predictions~\parencite{willard2020integrating}. If the \enquote{frame} is opened to include additional behaviors, the model will have to be retrained, and may not be able to incorporate new data~\parencite{denning2022context}. As a result, models must be well-constructed to start with and then maintained to account for changes in the environment or data.

In addition, traditional machine learning techniques can struggle in novel situations  because they lack both the understanding of context and the ability to generalize from previous experience~\parencite{krakowski2022artificial}. For example, an AI may play a brilliant game of chess without noticing the room it's playing in is on fire~\parencite{kasparov2017deep}. \textit{AlphaStar}, one of the most impressive examples of machine learning in a real-time combat environment required immense amounts of training, first on recorded human game play, and then additional \enquote{league play,} where models would compete against each other. Estimates are that the total amount of training time exceeded 400,000 TPU-hours~\parencite{wang_deep_2019}.  

It's not that we can't build AI that plays great chess. And it's not that we can't build great AI to fight fires~\parencite{dhiman2022firefighting}, but building an AI that can seamlessly and autonomously switch frames between these two tasks is completely beyond the current state of the art.
%\textit{DeepMind}'s AlphaStar project was limited to the game of \textit{Starcraft.} 

\subsubsection{Black Swans and Biased Data}
\label{sec:black_swans}

A \textit{Black Swan Event} is a highly unpredictable and rare occurrence that has potentially severe consequences. For example, the terrorist attacks of 9/11 and the global financial crash of 2008 could be considered examples. AI systems struggle to identify and deal with these events because they lack the ability to recognize patterns that are not present in the data they were trained on. The reason for this is that most data used for training is collected from systems that are functioning \textit{normally}. 

For example, it is relatively straightforward to create a training set of typical rush hour traffic by simply equipping cars with cameras and driving them around in cities known to have traffic problems. But this is only a partial solution that does not handle Black Swans. For example, in major evacuations such as those for hurricanes, traffic is often directed to use all available lanes. A self-driving car that is not trained for that possibility may behave in unpredictable ways. Without careful attention to the training data, a neural network can easily \enquote{learn} to ignore such corner cases. For example, a network can be trained to drive incapable of handling accidents, since they only happen in extremely rare instances~--~about 0.0002\% per mile driven~\parencite{usdot_traffic_2018}. 

%Bias is a similar, but more pernicious problem. Although we often read or hear about bias with regard to gender or race, bias is a fundamental property of all training data. For example, if an AI is tasked with predicting the level of combat activity in the US Army, it could learn a biased outcome based on raw historical data. For example. using the ratio of combat to non-combat roles for the US Army during operation IRAQI FREEDOM, an AI could achieve an accuracy score of over 96\% by assuming that soldiers in the US Army do not fight.~\parencite{mcgrath2007other, macrotrends_us_army_2019}.

To remedy this problem, it is important to obtain or create \textit{balanced} data sets. Such datasets can be created using simulation, which can create data that is too \enquote{clean.} Another option is to train \textit{shadow models} that attempt to predict the behavior of humans while performing the same task. Any deviation from the model's prediction is stored and used to create a more balanced data set for the following model which in turn is used to shadow the driver. This process has been used extensively in the development of autonomous automobiles such as Tesla~\parencite{liu2021analysis}. Even then, Black Swan events such as airplanes landing on the highway, animals wandering onto the road, or deliberate anti-AI sabotage have all been documented. Since models cannot adapt dynamically, they are destined to be one step behind the latest and greatest attack or exploit.

\subsubsection{Monolithic Models}
\label{sec:monolithic}
A singular, or monolithic, perspective on any matter is inherently biased, varying from a subtle inclination to a complete misjudgment of the matter at hand. The danger with a single viewpoint lies in the possibility that the leadership or decision-maker may become obstinate in their own perspective, impeding their ability to consider alternative outlooks. This rigidity may result in a narrow-minded or myopic decision that disregards a broader range of factors and potential consequences. Although such decisions may seem effective in the short term, it is imperative to remember that situations inevitably change, especially in dynamic environments like combat. %History is full of examples where leadership, sheltered from conflicting views made disastrous decisions, ranging from the French at the Battle of Agincourt to the inability of US forces to fully defeat the Taliban insurgency in Afghanistan~\parencite{kolenda2019slow, waldman2013system}.

In the realm of AI, a similar issue emerges. Many extensive AI systems rely on a single architecture and dataset, with sophisticated models proving costly to train. For instance, the \textit{AlphaStar} model is estimated to have required \$12 million in processing time for its creation~\parencite{wang_deep_2019}. Consequently, developing and testing additional models with equivalent capabilities becomes financially unjustifiable for the marginal gain. Regardless of alternative architectures or data, the odds of a model being significantly better or worse remain low. Instead, these large models can be \textit{finetuned} to exhibit different behaviors, though their underlying structure stays untouched. As a result, seemingly distinct models may possess shared vulnerabilities. 

This vulnerability exists because models are evaluated on how well they meet an \textit{objective function}. It may be predicting the most likely next word in a sentence, or it can be winning at \textit{AlphaStar}. In all cases, the model is attempting to optimize its behavior in response to its inputs. If model becomes too optimized, particularly with respect to attributes that are not easy to quantify, it can become brittle and vulnerable to adversarial attacks~\parencite{giddings2022optimizing}. These vulnerabilities are often undetectable. By training multiple models using different objective functions, developers can create a robust \textit{ensemble} of models and reduce vulnerability while also increasing potential flexibility in unforeseen situations.

The key to robustness in AI systems is diversity. Diversity of data, algorithms, models, and people. In the case of AI models, it is important to have multiple models that have been trained differently in order to reduce the chances of relying solely on a single perspective. This is especially important when the goal is to create a system that can generalize to a wide variety of situations, as multiple models combined with human operators would provide the largest possible pool of data and experiences to draw from. If a single model fails, the other models in the ensemble can be selected to continue operation.

Finally, resilient systems must also possess the ability to fail gracefully. This means that when a component such as a model fails, the \textit{system} should be able to adjust and continue without significant disruption. The concept of graceful degradation is an important one for combat AI systems, as it can help ensure that these systems are able to perform effectively under the widest range of conditions. By incorporating diversity, adaptivity, and the ability to fail gracefully, AI systems can be better equipped to handle the challenges of the battlefield.

==> text2/background.tex <==
\section{BACKGROUND}

Current AI systems can be divided into two categories: \enquote{Strong AI}, as-yet unrealized systems that can think and act~\parencite{ibm:what_is_ai_2023}, and  \enquote{Weak,} or \enquote{Narrow AI}, which are broadly available systems that can complete specific tasks with a high degree of accuracy~\parencite{devedzic2022identity}. Examples of Narrow AI include self-driving cars, robotic arms in factories, and voice recognition systems. However, there are still many areas where these systems struggle to be effective and reliable, such as decision making in complex environments or interactions between humans and autonomous agents~\parencite{ng2020strong}. Previous approaches such as \enquote{Expert Systems} depended on symbolic processing and rule-based systems. Such techniques are now known as \enquote{Good Old-Fashioned AI} (GOFAI), and can be considered as a (narrower) subset of Narrow AI~\parencite{devedzic2022identity} that does not use deep neural networks. In some respects, these distinctions don't matter with respect to how we as humans interact with these systems. They work at speeds and scales that we cannot. We tend to place excessive trust in their outputs, particularly when our cognitive bandwidth is compromised in some way.

Nonetheless, humans and machines must work together effectively in the extreme conditions exemplified by combat. So in this section, we will first discuss the areas where current state-of-the-art AI systems struggle to be effective, reliable, and accurate. We will then examine approaches that have been shown to result in more effective and reliable human/autonomous system pairing.

\input{text2/AI_problems.tex}
\input{text2/human_problems.tex}

\begin{comment}



\TODO{Delay this} In the context of AI combat this means that the most robust and resilient systems should consist of diverse teams of operators that can select from a set of models to choose -- and if needed dynamically change -- on the fly. This combination of diverse operators and model ensembles combine to create a level of group cognition that should be more powerful and effective than any individual model or operator.

The challenge with this approach is that it requires a level of trust and cooperation between different operators to ensure that they can quickly select the right models and strategies for any given situation, in lieu of relying on a single (biased) view and its associated options. To support these teams, new types of interfaces and controls should be considered, which we will discuss next.

%Tank crews as group problem solving as a single entity


\end{comment}





==> text2/geopolitical.tex <==
\subsection{Geopolitical Implications}

% Prompt: Write a concluding essay for a paper on the geopolitical implications of using AI in the military. The argument is that diverse teams monitoring ensembles of models ensure the highest levels of performance and flexibility, while structurally "building in" ethical behavior. Further show that an effective application of combat AI supervised by diverse teams places authoritarian and autocratic regimes in a bind. Such governments are threatened by diverse points of view, so would be starved for the kind of sophisticated AI operator that is needed for resilient, effective use of combat AI. While on the other hand, democracies tend to cultivate such subgroups from which to draw from. As such, governments that are structured on dominance of the homogeneous  few over a subservient heterogeneous population are placed where the diversity that supports effective combat AI is unavailable to them. To compete on the battlefield, they will have to open their societies, which may cause more beneficial effects than any weapons system, no matter how sophisticated.

The approach described in this paper may have significant geopolitical implications. Diverse teams, monitoring ensembles of models, can ensure the highest levels of performance and flexibility in AI combat. Such teams bring different perspectives, experiences, and expertise, which helps to identify and effectively react to latent, unforeseen  biases and limitations in the models, particularly when the systems need to operate outside of the domain they were trained for. Diverse teams  also \enquote{build in} ethical behavior by incorporating lived experience into the design and use of AI systems.

Effective application of combat AI supervised by diverse teams may place authoritarian regimes in a difficult position. Such governments are often threatened by diverse points of view and may be unable to cultivate the kind of sophisticated AI operators needed for effective use of combat AI. Democracies, on the other hand, tend to have more diverse and inclusive societies, providing a larger pool of potential AI operators. This could give democracies a significant advantage in using AI in combat and other scenarios~\parencite{arendt1951origins}.

For example, a restrictive, low-diversity government may have strict controls on the education and career paths of its citizens, leading to a homogeneous group of AI operators who may lack the necessary skills and experiences to effectively exploit combat AI. In contrast, a dynamic, high-diversity government may have a more open and inclusive education system, leading to a diverse group of AI operators with a wide range of skills and expertise~\parencite{zhao2011impact}. This diversity of perspectives and experiences can be particularly valuable in the rapidly changing and complex environment of modern warfare~\parencite{clearfield2018meltdown}.

% As a result, governments that are structured on the dominance of a single group over subjugated minorities or that fail to embrace diversity in their social structure may find themselves at a disadvantage when it comes to using AI in the military. %To compete on the battlefield, they may have to open their societies and embrace diversity, which could have more beneficial effects than any weapons system, no matter how sophisticated. 

==> text2/human_problems.tex <==
\subsection{Human Limitations}
\label{sec:human_problems}
%\TODO{Humans have their own set of problems. Confirmation bias, principle, of least effort, etc. Fortunately, they don't overlap!}

The problem with intelligent systems is not just with the machines, it is with humans as well. At each level of interaction, human-in-the-loop, human-on-the-loop, or interacting with decision aids, we as humans tend to trust systems that are correct most of the time. This is known as the \textit{automation conundrum}, where the more reliable and effective a system is, the less likely it is that a human operator will elect to take over control when needed~\parencite{endsley2017here}. 

\subsubsection{Normal Accidents}
\label{sec:normal_accidents}

Charles Perrow established the concept of \enquote{Normal Accidents} \parencite{perrow2011normal} as a property of high-risk systems based on his analysis of the Three Mile Island partial meltdown in 1979. Normal Accidents are unpredictable, yet inevitable combinations of small failures that build upon each other within an unforgiving environment. Normal accidents include catastrophic failures such as chemical plant explosions, airplane crashes, and stock market collapses. Though each failure is unique, all these failures have common properties:

\begin{enumerate}
	\item The system's components are tightly coupled. A change in one part has rapid consequences elsewhere.
	\item The system is densely connected, so that the actions of one part affects many others.
	\item The system's internals are difficult to observe, so that failure can appear without warning.
\end{enumerate}


Battlespace systems are complicated, consisting of numerous components integrated in complex
physical, electronic, and software webs. They are high risk, both at the individual level, where elements can be lost to combat and other attrition, and in a broader context, where misallocation of resources during an emergency could result in large scale suffering or death. 

Recall the Patriot Missile batteries described in the introduction. Because the operators did not have visibility to the internals of the system, they were unable to determine quickly if the computer's recommendation was correct. Due to a simple display obscuring great complexity, friendly aircraft were tragically destroyed.

In order to ensure the highest levels of reliability and performance, it is essential that the combat AI systems are designed and built from the ground up with usability in mind. 

% This involves taking a holistic approach to system design that considers the entire system as an integrated whole and not just individual components.

% User interface is essential in order to ensure that the system is understandable and manageable by the operators.

The key elements of usable design include user interface, resilience, and redundancy. Good user interfaces allow operators to understand the salient characteristics of the system without being overwhelmed. Resilience allows a system to be damaged in places and still be able to function, so that if one component of the system fails there are alternative  means of achieving the same goal. In those areas where it is not practical to engineer in resilience, critical elements must be robust and able to survive attempts at disruption. Finally, redundancy should be considered and implemented wherever possible. This ensures that if one element of the system fails, there will be a backup in place to take its place.

\subsubsection{Human in/on the Loop}
\label{sec:human_loops}

If a human operator has sufficient warning as to when they may  need to take over from a machine, they can acquire the situational awareness necessary to understand the context of what is happening and take \textit{effective} control. Without this prior knowledge, the operator is likely to be overwhelmed and unable to take appropriate action.

Low situational awareness occurs due to three primary mechanisms~\parencite{endsley2017here}:

\begin{enumerate}
    \item \textit{Changes in information presentation with automation}: Often, the substitution of automation for human interaction also includes the removal of critical information from the user interface. For example, many autopilot systems do not provide tactile feedback to pilots through the controls when engaged, as in the case with the Airbus A320/330/340 sidestick controllers~\parencite{billings1991human}. This loss of \enquote{ambient} information requires additional cognitive activity on the part of an operator during an emergency -- precisely when that time does not exist. Unfortunately, reducing the information available to the operator as the level of automation increases is a common problem in such systems.
    
    \item \textit{Operator monitoring, vigilance and trust}: Human vigilance of automated systems, including AI, is necessary to ensure that they are functioning properly. However, it is important to note that people may not be willing or able to pay attention to the system for long periods of time due to complacency or overreliance on the system. Additionally, trust in the automation leads to a decrease in vigilance, further exacerbating the problem.
    
    \item \textit{Operator engagement}: It is harder for operators to understand a task when they are passively monitoring automation compared to when they are actively processing information to manually perform the same task. Active engagement requires people to use information in a way that goes beyond passive reading or listening; it enables them to better understand relevant tasks and retain more critical information. It is more difficult for operators to understand those tasks while passively monitoring an automated system. Such passive monitoring diminishes situational and presents a challenge for effective human-autonomy interactions.
\end{enumerate}

The  more reliable the automation, the less likely the human operator will elect to take over manual control when needed.  As individual functions are automated and the reliability of the automation increases, less attention will be paid to those functions and situational awareness of the human operator will deteriorate. This increases the likelihood of an \textit{out-of-the-loop} (OOTL) error in the case of unexpected automation transitions~\parencite{endsley2017here}.

% I want/need an operator to be tied into that system. Part of this teaming is queuing or identification of anomally. That is part of situational understanding. You are operating in an area on a daily basis. Busy area, you've come to know the people who own the local establishments. If those people do not show up at expected times, that should provide a contextual clue to operation.

% When you add people to manage higher levels of abstraction and provide them tools that support those higher levels (such as viewing anomalies over time) this integrates the operator into the system at a level where they can provide context rather than reacting to individual decisions when the system fails.

\subsubsection{Decision Aids}
\label{sec:decision_aids}

A related problem with human behavior  occurs with relation to \textit{decision aids}. In these applications, the human user is provided with information and recommendations to make optimal decisions in the minimum amount of time. %This is the fundamental problem with the Patriot friendly fire scenario. %The AI agent might consider a variety of factors, including the user’s preferences, the cost of decisions, the amount of time available, and the potential consequences of the decision.

Decision aids have been used in domains such as healthcare, finance, criminal justice, hiring, and more~\parencite{lai2021towards}. AI-based decision aids have been shown to be capable of improving decision-making accuracy, and reducing decision-making time. 

Numerous studies have shown that when the advice from a decision aid is correct, people are more likely to make correct decisions. However, when the advice is faulty or incomplete, people perform worse than if they had received no decision advice at all. This behavior can be catastrophic in combat situations, particularly if users need to compare the system’s recommendation with other information to decide whether or not to agree with it~\parencite{olson1999supporting}.

Studies have also shown that when users are presented with a decision aid that provides wrong advice, they tend to either accept the advice without verifying it, or they check the relevant information but \textit{still follow the wrong advice}. For example, a study looking at the consequences of three automated aids for the support of a supervisory control task found that half of people who accepted incorrect system advice failed to verify the recommendation, and the other half apparently checked all the relevant information but still implemented the incorrect decision. Whether the system only recommends, with the human making the ultimate decision (management by consent), or the system makes the selection and implements it unless the human vetoes (management by exception) makes little difference to error recovery times~\parencite{manzey2012human}.

\subsubsection{Information Displays}
\label{sec:information_displays}

Modern warfare can be dynamic, kinetic, and overwhelming. It can also be tedious and boring between those kinetic events. In the past, strategy and tactics focused mostly with how human beings used technology and the physical environment to achieve dominance over an adversary. However, with the modern battlefield being increasingly saturated with data and technology, this has become much more difficult. 

At present, to manage the deluge of information and avoid overwhelming operators, designers are incorporating AI to condense and interpret massive data sets, displaying the results in a way that is quickly understandable even under extreme stress (refer to Figure~\ref{fig:md_ops} for an illustration). Additionally, the AI might suggest actions that the operator can accept or decline. However, this approach presumes that the AI is making the best decisions for the situation at hand. To ensure that AI systems are indeed making appropriate choices, the idea of \textit{explainable AI} (XAI) has been proposed. XAI is designed to provide clear rationales for the AI's decisions or advice. 

\begin{figure}[!htbp]
    \centering
    \fbox{\includegraphics[width=30em]{figures/md_ops}}
    \caption{\label{fig:md_ops} U.S. Army in Multi-Domain Operations 2028~\parencite{multi_domain_2019}}
\end{figure}

As seen in the previous section, the effort required on the part of the human operator to understand the explanations adds to the cognitive load so that the ability to understand and trace back decisions are not sufficient to avoid making incorrect decisions~\parencite{janssen2022will}. Almost inevitably, even experts follow the recommendations of the system, even when they are wrong~\parencite{Vasconcelos_Explanations_2022}.

In apparent disregard for this observed tendency for users to uncritically accept system recommendations, there is an increasing trend for automated systems to facilitate decision making. The need for humans to understand their capabilities, limitations, and interactions with other systems is critical. The need to protect these systems from malicious actors is also increasing. The complexity and opacity of these systems make it difficult to understand their behaviour and potential vulnerabilities. Automated systems can be vulnerable to cyber-attacks and exploits. 

% A new role is needed to understand if these increasingly complex systems are behaving as intended. 

Paradoxically, we may be able to find useful insights into our future systems by looking at history.


==> text2/introduction.tex <==
\section{INTRODUCTION}
\begin{comment}
    \begin{displayquote}
        \textit{The Commission is not glorifying the prospect of AI-enabled warfare. But new technology is almost always employed for the pursuit of power. In light of the choices being made by our strategic competitors, the United States must also examine AI through a military lens, including concepts for AI-enabled autonomous operations.}~\parencite{schmidt2019national}
        
        \hfill -- National Security Commission on Artificial Intelligence (Interim)
    \end{displayquote}
\end{comment}

\TODO{Something about the perceived risk of LAWS being sand in the gears for decision making. Ideally, what is needed is an effective, generalizable template that can provide an ethical framework and speed approval of LAWS systems.}

The paradigm of human involvement in lethal AI combat systems seems to be headed towards a reckoning. There are now nation-states that appear to be developing combat AI systems that have no human involvement other than the activation of the weapon, such as loitering munitions that look for armored vehicles within a specified set of coordinates. 

% If it turns out to have misidentified a bus full of fleeing refugees as an armored personnel carrier, that's too bad.

%The belief that to have competitive AI on the battlefield, we need to make hard ethical choices is captured perfectly by the above quote from the interim report by the NSCAI. 

To address the ethical considerations posed by these AI-enabled weapons, the DoD updated the its directive on \enquote{autonomy in weapons systems} in 2023~\parencite{dod:3000-09_2023}. In 2022, the White House released a \enquote{Blueprint for an AI Bill of Rights} that expanded on those DoD principles~\parencite{wh:AI_BillOfRights_2023}. While work is ongoing at the highest levels of the United States government to address these issues, to date the DoD Directive 3000.09 is the only \textit{formal policy} addressing AI weapons. 

%\TODO{Note that 3000.09 paragraph 3b states that people use or authorise autonomous systems must me in accordance with the Law of War, which states that \enquote{War crimes are those violations of international humanitarian law (treaty or customary law) that incur individual criminal responsibility.}}

% DoD Directive 3000.09 [64] established DoD policy regarding autonomous and semiautonomous weapons systems and guidelines to minimize its attendant ethical and practical risks. 

% \enquote{This policy extends to autonomous and semiautonomous, manned and unmanned, and lethal and nonlethal systems. It is important to note that this directive institutes policies and reviews and assigns responsibilities for its own implementation. \textit{It does not technically allow or disallow any specific practice in AI} or autonomy but sets policies where systems be designed to allow commanders and operators exercise \enquote{appropriate levels of human judgment} over the use of force.}

A 2022 Technical report by the Defense Technical Information Center (DTIC) states \enquote{a human in the loop may be necessary and practical in situations where human life is actually or potentially at stake [...] The human operator then retains the capacity and responsibility to veto or override the robot’s decisions as needed.}~\parencite{chakour2022SOAR} Similarly, directive 3000.09 states that autonomous systems \enquote{will have been demonstrated to allow commanders and operators to exercise appropriate levels of human judgment} (Section 4.1.D.1).

% Any fielded system would involve a human operator monitoring the behavior of the autonomous system and will at the least have \enquote{veto power} if a system incorrectly identifies a target~\parencite{chakour2022SOAR}. 

% To prevent this type of tragedy, the United States and other Western countries should strive to develop autonomous systems that are \textit{always} supervised by humans. Any fielded system would involve a human operator monitoring the behavior of the autonomous system and will at the least have \enquote{veto power} if a system incorrectly identifies a target~\parencite{chakour2022SOAR}. 

An example of such a veto is described by Paul Scharre in his book \textit{Army of None}, where a church was mistaken for an early warning radar and engaged using a remotely-operated AGM-130 missile fired from an F-15E. A mere three \textit{seconds} before impact, the missile operator identified the error and ditched the missile in a field by the church~\parencite{scharre2018army}.

AI systems can recommend actions that human users may choose to adopt or reject. However, humans tend to favor accepting machine recommendations, even if they are incorrect, when the system has a high success rate. This was evident in the 2003 Gulf War, where the \textit{functioning} Patriot Missile batteries destroyed two friendly aircraft. The radar system detected an incoming object and recommended firing at a target identified as a missile. The operators agreed with the recommendation and fired at a Tornado GR4A fighter, which was landing, resulting in its destruction and the death of its crew~\parencite{scharre2018army}.

AI weapons promise greater accuracy and speed of response than those controlled by human operators. This raises a dilemma for those responsible for developing weapons in accordance with International Humanitarian Law (IHL), that requires a human be responsible for the use of lethal force.  On one hand, AI weapons must be designed so that humans always have the ability to act as an ethical fail-safe. On the other hand, militaries around the world are currently racing to develop fully autonomous weapons that can take action without any human input. The conventional wisdom is that a human-in/on-the-loop system cannot compete with unconstrained AI in unpredictable battlefield environments.

In the case where the operator is \enquote{in the loop,} directly interacting with the AI, the risk is that the operator may not have adequate time to make ethical decisions, leading to potential violations of IHL. On the other hand, when the operator is \enquote{on the loop,} or supervising the behavior of the system, the risk is that the AI may be able to outpace the human operator's ability to react quickly enough to prevent a violation of IHL. This presents a difficult dilemma for combat AI systems: how to balance the need for speed and efficiency with the need for ethical compliance.

 Given that combat systems are functioning in shorter timeframes and over broader scales, this problem appears to be intractable. Human beings seem incapable of keeping pace with AI
weapons, yet for systems to behave in ethical ways, they \textit{must}. In the following pages, we propose an approach to intelligent combat systems that shifts the human responsibility from operating the system to a higher level interaction with AI models. This would allow humans to use their advantages in diversity, contextualization, social interaction, and creativity to govern the \textit{higher-order} behavior of intelligent combat systems. In this way, humans provide the large scale, long term awareness, while the machines provide the speed of reaction. 

This approach enables the development of combat systems that are ethical, operate at machine speed, and are capable of adapting to a broader range of dynamic battlefield conditions than any AI system could handle on its own.


==> text2/symposim_abstract.tex <==
\begin{abstract}
    
    This presentation will explore the changes that AI is having on the nature of combat. We will first look at the current practice where AI substitutes for the human for most tasks, and the human provides a final check or veto. We show that this approach is brittle and tends to expose weaknesses of both AI and humans. We then explore an alternative approach where complementary human and machine abilities are blended. Using the historical example of War Elephants, used as a type of lethal autonomous weapons system for thousands of years, as well as more recent examples from the conflict in Ukraine, we show how autonomous weapons systems can be more effectively managed by specially trained AI Operators. 
    
    The AI Operators are responsible for watching over the AI system, and detecting when the AI fails to behave in accordance with the warfighter's intent. By blending the human capacity for social thought, context changing, and creativity with the AI's speed and precision, the AI operators can quickly and efficiently detect anomalies in the AI's behavior. When a potential problem appears, the AI operators can intervene in the system and take corrective action. The AI operators must be trained to recognize when the AI system is making decisions that are not in line with the warfighter's intent and understand how to intervene.
    
    Next, we will discuss the need for diverse model ensembles and the training and equipping of AI Operators.  We will discuss how these proposed human/machine teams will possess the capability to act outside of the domain that they were developed and trained for.
    
    We discuss a path to achieve machine-speed/machine-scale combat where the AI is operated by diverse Operator teams that watch for patterns of behavior to assess the system's performance. This approach enables the development of combat systems that are inherently ethical, operate at machine speed, and are capable of responding to a broader range of dynamic battlefield conditions than any AI system could achieve on its own.
    
    In accordance with the recommendations of the National Security Commission on Artificial Intelligence, we conclude that a human-centered approach, in which the strengths of both humans and AI are balanced, ensures that AI models are always used in accordance with the principles of international humanitarian law, and that ethical behavior is an enhancement of performance, not a hindrance.


\end{abstract}


==> text2/things_that_work.tex <==
\section{When AI Works}

Humans and AI can complement each other in tasks requiring comprehension, creativity, and innovation. Self-driving cars excel in good weather on limited-access roads, while language models can produce realistic text without understanding facts from fiction. AI can diagnose diseases more accurately, quickly, and cost-effectively than before, but it is not without flaws, such as misinterpreting X-rays~\parencite{majeed2020issues}. Under appropriate conditions, AI can provide insights that enable humans to make better choices.

Humans can use their creativity and innovation to come up with new ideas and solutions that AI can't. We can also understand the nuances and context of a situation that AI misses, which can be critical in decision-making. Lastly, humans perform best in groups, where each person brings different perspectives and skills, providing a \textit{depth of understanding} that current AI can appear to mimic, but cannot replicate.

Complementation, or mutual reinforcement, has been shown to enhance the effectiveness and reliability of human/autonomous systems. The game of chess provides an example, where a human-machine pair outperforms each component alone~\parencite{scharre2016centaur, kasparov2017deep}. Unlike substitution, where the most capable component is used in isolation, complementation combines multiple elements to produce a more effective whole. Substitution systems are limited by their weakest component, as discussed in Section~\ref{sec:ai_problems}.

We will now discuss how complementation may be applied to combat systems with respect to the particular strengths and weaknesses of humans and AI. There is an accepted view of human/AI teaming where  humans bring their creativity and strategic thinking to bear, and AI can provide processing speed and power. We believe that this view is incomplete and overlooks potential areas of mutual reinforcement. 

\subsection{Human-AI Complementation}

The primary goal of human/AI teaming is to create a system that can outperform any individual component. The key to this type of teaming lies in understanding the strengths and weaknesses of both humans and AI, and then exploiting areas where they complement each other. 

Local, rapid interaction with AI has proven effective in producing precision results, as demonstrated in reports on Ukrainian drone combat~\parencite{Wyrwa2022Wojna}. To fight the Russian invasion, the Ukrainian government has enlisted private companies to develop technology, resulting in diverse drone systems with non-GPS navigation and trained image recognition systems capable of identifying camouflaged vehicles. These drones can carry four RKG-1600 anti-tank munitions modified as small bombs.

The human operator guides the drone to the target region. As it flies, the drone's cameras identify potential targets, such as tanks with a confidence score (Figure~\ref{fig:drone_tank_id}). It can also misidentify, for example, a clump of trees as a camouflaged vehicle (Figure~\ref{fig:drone_tree_id}). It is up to the operator to make the determination and begin the engagement.

\begin{figure}[!htbp]
    \centerline{
	\centering
        \begin{subfigure}{.5\textwidth}
    	\centering
    	\fbox{\includegraphics[height=10em]{figures/drone_tank_id}}
    	\caption{\label{fig:drone_tank_id}Correct drone tank ID}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
    	\centering
    	\fbox{\includegraphics[height=10em]{figures/drone_tree_id}}
    	\caption{\label{fig:drone_tree_id}Incorrect drone tank ID}
     \end{subfigure}
     }
\end{figure}

The drone maneuvers to be above the target and then drops a munition. Based on the impact and the position of the target, the drone adjusts its position if needed and drops the second munition when often results in a hit on the target, ideally leaving two more munitions for another engagement. 

The human operator interacts dynamically with the drone, verifying target identification before initiating an attack. This allows the AI to be more sensitive, but also keeps the operator involved in the process. During an attack the AI does not have to be perfect because the human verifies. The drone operates in a constrained envelope near the target, minimizing stochastic error. 

In contrast, the Iranian-made Shahed 136 drone used by Russia in Ukraine lacks regular human input, relying on pre-programmed GPS coordinates and often used in swarms. This has resulted in civilian fatalities in Ukraine, Yemen, Syria, and Iraq~\parencite{enwiki_Shahed_2022}. The AI's inability to make real-time adjustments increases the risk of collateral damage.

In both cases, the drones have the capacity to be completely autonomous. In the case of the Ukrainian drones, the continual interaction of the operator and the useful user interface means that the drone is largely operated in an ethical manner, in accordance with international humanitarian law (IHL)~\parencite{un2018laws}. Reducing the interaction with the corresponding increase in autonomy creates a weapon in the Shahed 136 that violates these laws and is likely to have been part of operations that are war crimes.

It is important to note that both of these systems have been effective in combat. The Ukrainian system does not suffer from being ethical, and the Iranian system does not gain a dramatic combat advantage from its increased autonomy.  The difference between these two systems is the potential for collateral damage, with the Iranian system having a higher potential for such damage.  This illustrates the importance of keeping an ethical approach to AI-driven weapons, as there is no need to sacrifice ethical considerations for effectiveness. 


